Understanding the Challenges and Assisting Developers with Developing Spark Applications

To process data more efficiently, big data frameworks provide data abstractions to developers. However, due to the abstraction, there may be many challenges for developers to understand and debug the data processing code. To uncover the challenges in using big data frameworks, we first conduct an empirical study on 1,000 Apache Spark-related questions on Stack Overflow. We find that most of the challenges are related to data transformation and API usage. To solve these challenges, we design an approach, which assists developers with understanding and debugging data processing in Spark. Our approach leverages statistical sampling to minimize performance overhead, and provides intermediate information and hint messages for each data processing step of a chained method pipeline. The preliminary evaluation of our approach shows that it has low performance overhead and we receive good feedback from developers.

==> Makefile <==

default: paper 
coall:
	co RCS/*

ciall:
	ci -u *.tex
	ci -u *.eps

bib: paper.bbl

paper.bbl: *.tex paper.bib
	latex paper
	bibtex paper
	latex paper

paper.ps: paper.dvi
	dvips -P cmz paper.dvi -o paper.ps -t letter

paper.dvi: *.tex paper.bbl
	latex paper
	latex paper

paper.pdf: *.tex
	pdflatex paper
	pdflatex paper
mpost:
	mpost -tex=latex overview.mp

	
paper: *.tex
	pdflatex main 
	bibtex main
	pdflatex main
	pdflatex main
	@echo "**********************************************************************"
	@echo "***	Did you spell-check your commit?		     ********"
	@echo "***	Did you spell-check your commit?		     ********"
	@echo "***	Did you spell-check your commit?		     ********"
	@echo "***	Did you spell-check your commit?		     ********"
	@echo "***	Did you spell-check your commit?		     ********"
	@echo "***	Did you run grammarly on your commit?		     ********"
	@echo "**********************************************************************"

purge:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps \
		overview.mps\
		paper.pdf

clean:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
		*.fls \
		*.fdb_latexm \
                paper.ps




==> texFiles/background.tex <==
%\peter{Here, we should talk about a few things. First, what is Spark in general: how it is the most popular solution, how the APIs are designed (fluent API, methodal programming), distributed computing, lazy evaluation. This should take maybe 0.25 to 0.5 page at most. After this, we provide a brief discussion on which API sets we include and why (e.g., why not RDD and why dataset). Then, we discuss the current log/debugging that is provided by Spark. Production monitoring/debugging, what is available (describe what they have, and say what is missing). We provide a brief discussion on what we provide, and this is bridging the gap between the current Spark design and its monitoring/debugging}



\begin{comment}



Spark is a distributed cluster-computing framework that can execute the computation in parallel in a cluster. When using Spark, developers do not need to worry about the implementation details of distributing the computation across worker nodes, since Spark abstracts the underlying parallel computation and cluster management from developers. Spark provides APIs for three programming languages: Scala, Java, and Python. In this paper, we focus our study and implementation on Spark's Python API(PySpark), and the concepts are applicable to the APIs in other programming languages. For the version of our experimental software, the Python version is 3.7.3 and Spark version is 2.4.4. To process data, Spark provides three abstractions for distributed data: RDD (resilient distributed dataset), DataSet, and DataFrame. RDD is an immutable distributed collection of data elements that can be operated in parallel. After Spark 2.0, RDD is replaced by Dataset and DataFrame, which provide richer APIs and better performance optimization. DataSet and DataFrame are both an abstract for a distributed collection data, whereas DataFrame further groups the data into named columns. Note that PySpark only supports DataFrame due to its popularity. Below, we focus our discussion on DataFrame.


Spark APIs leverage two important concepts in the design: {\bf method chaining} and {\bf lazy evaluation}.
Method chaining is used to ensure data immutability (i.e., DataFrame objects are immutable to avoid concurrency issues) and allows developers to create a data processing pipeline by chaining multiple data processing methods. For example, developers can call \texttt{dataFrame.filter(x $>$ 3).dropDuplicates().sort()} as a chain.
By chaining the three data processing methods (i.e., \texttt{filter}, \texttt{dropDuplicates}, and \texttt{sort}), each method would return a new DataFrame object that is used as the input for the next method. The final returned DataFrame object will have the values larger than three being filtered, duplicates removed, and sorted. Such a method chaining also provides an intuitive way for developers to combine multiple data processing methods.

To optimize the performance of the chained methods, Spark employs lazy evaluation for optimization. There are two types of methods: transformation and action. For example, \texttt{filter} is a transformation method and \texttt{count} is an action method (i.e., return the number of rows in the data). All the transformation methods are lazily evaluated until an action method is called. When an action method is called, similar to compiler optimization, some intermediate data processing steps in Spark may be optimized, combined, or even eliminated to improve performance. If no action method is called, Spark would not execute any transformation method. For example, \texttt{dataFrame.filter(x $>$ 3)} will not really filter the data immediately, unless an action method is called, like \texttt{count}. Then Spark will start to filter data and calculate the number of rows of the filtered data.

Even though method chaining and lazy evaluation provide developers with the flexibility in using the data processing methods and the benefit for performance optimization, development challenges may exist. For example, developers may not be able to know how the data is transformed in each step of the chained methods, which may increase debugging difficulties. However, forcing Spark to return and retrieve the intermediate information of each step can invalidate lazy evaluation and cause significant performance overhead (e.g., the data needs to be collected from all the worker nodes for every step). Hence, in this paper, we first conduct an empirical study on the development challenges that developers encounter by analyzing Spark-related questions on Stack Overflow. Based on our findings, we propose and design an approach, called \tool, which assists developers with debugging Spark applications by providing intermediate data processing results without invalidating the lazy evaluation. %In addition, \tool has a low performance overhead, and through a user study,

\end{comment}

%all data processing methods for data processing are transformation. The methods that are used to do basic data processing on the dataframe are: \texttt{Filter}, \texttt{dropDuplicates}, \texttt{distinct}, \texttt{distinct}, \texttt{dropna}, \texttt{fillna}, \texttt{drop}, \texttt{join}, \texttt{withColumn}, \texttt{sort}.



%Python does not have the support for the Dataset API. In pyspark, only RDD and DataFrame are available. Spark DataFrame is immutable. For DataFrame, there are two types of operations: transformation and action. The transformation will return a new DataFrame from the existing DataFrame. The action will return a value to the driver program after running a computation on the DataFrame. For example, \texttt{Filter} is a transformation method in DataFrame, this method will filter rows using the given condition and return a new DataFrame. \texttt{count} is an action method in DataFrame, this method will return the number of rows in the DataFrame to the driver program.

%It should be noted that all transformation on Spark are lazy. Transformation will not execute immediately. Spark maintains the record of which transformation operation is being called through DAG(Directed Acyclic Graph). The transformations are only computed when an action is called. For example, When a dataframe calls the filter method to filter data, the filter method will not be executed immediately, until the dataframe calls an action method, such as count, then the calculation including filter and count will start. This computation mode is call lazy evaluation. \wang{we should use lazy evaluation in the rest of paper.}

%Although the calculation process of transformation is not visible to develoeprs, Spark can see all the methods that need to be calculated through this mode, and integrate the methods into different stages to execute, and achieve the best performance.

%\peter{@Shaowei, please see if we need to keep it here or integrate some to implementation}For DataFrame, all methods for data processing are transformation. The methods that are used to do basic data processing on the dataframe are: \texttt{Filter}, \texttt{dropDuplicates}, \texttt{distinct}, \texttt{distinct}, \texttt{dropna}, \texttt{fillna}, \texttt{drop}, \texttt{join}, \texttt{withColumn}, \texttt{sort}.
%Deduplication can effectively reduce the data set and simplify the dataset to improve performance. The \texttt{dropDuplicates} and \texttt{distinct} both will return a new DataFrame with duplicate rows removed. The difference is that \texttt{dropDuplicates} can deduplication\hl{what is the meaning?} based on the selected columns. \texttt{dropna} and \texttt{fillna} are essential methods in data cleaning. \texttt{dropna} will return a new DataFrame by removing the rows with null value. \texttt{fillna} will return a new DataFame by filling in the null value using the selected value. The \texttt{drop} will return a new DataFrame that drops the selected columns. \texttt{join} is also a frequently used method in Spark. \texttt{join} will join two DataFrame based on the assigned condition. \texttt{withColumn} will return a new DataFrame by adding a column. If the name of new column is same as the old one, the new column will replace the existing column that has the same name. \texttt{withColumn} is the most common method for data processing on spark. Because the dataframe is immutable, developers who wish to perform any operation on a column of data in the dataframe need to use this method. \texttt{sort} will return a new DataFrame that is sorted by the assigned columns.



%DataSet is a distributed collection of data. DataFrame is a distributed collection of data grouped into named columns.

%Spark is a distributed cluster-computing framework which can execute the computation in parallel in a cluster. When using Spark, developers do not need to worry about distributing the computation across worker nodes, since Spark abstracts the underlying parallel computation and cluster management from developers. To process data, Spark provides several data abstraction for developers: RDD (resilient distributed dataset), DataSet, DataFrame. RDD is an immutable distributed collection of data elements that can be operated in parallel. After Spark 2.0, RDD is replaced by Dataset and DataFrame, which provide richer APIs and better performance optimization.

%of developers' data. The RDD partitions across nodes in developers' cluster and can be operated in parallel. DataSet is a distributed collection of data. DataFrame is a distributed collection of data grouped into named columns. RDD is the main programming interface of Spark before Spark 2.0. After Spark 2.0, RDDs are replaced by Dataset and Dataframe, which is richer optimizations and has better peformance. Spark mainly supports three programming languages: Scala, Java, Python. Spark also provides an R package that provides a light-weight Spark's methods from R. DataSet and DataFrame is available in Java, Scala.




%. Each Spark application has a driver program that is defined by users and executes various parallel operations on a cluster.

%To process data, Spark provides several data abstraction for developers: RDD, DataSet, DataFrame. RDD (resilient distributed dataset) is an immutable distributed collection of elements of developers' data. The RDD partitions across nodes in developers' cluster and can be operated in parallel. DataSet is a distributed collection of data. DataFrame is a distributed collection of data grouped into named columns. RDD is the main programming interface of Spark before Spark 2.0. After Spark 2.0, RDDs are replaced by Dataset and Dataframe, which is richer optimizations and has better peformance. Spark mainly supports three programming languages: Scala, Java, Python. Spark also provides an R package that provides a light-weight Spark's methods from R. DataSet and DataFrame is available in Java, Scala.

\begin{comment}
Python does not have the support for the Dataset API. In pyspark, only RDD and DataFrame are available. Spark DataFrame is immutable. For DataFrame, there are two types of operations: transformation and action. The transformation will return a new DataFrame from the existing DataFrame. The action will return a value to the driver program after running a computation on the DataFrame. For example, \texttt{Filter} is a transformation method in DataFrame, this method will filter rows using the given condition and return a new DataFrame. \texttt{count} is an action method in DataFrame, this method will return the number of rows in the DataFrame to the driver program.

It should be noted that all transformation on Spark are lazy. Transformation will not execute immediately. Spark maintains the record of which transformation operation is being called through DAG(Directed Acyclic Graph). The transformations are only computed when an action is called. For example, When a dataframe calls the filter method to filter data, the filter method will not be executed immediately, until the dataframe calls an action method, such as count, then the calculation including filter and count will start. This computation mode is call lazy evaluation. \wang{we should use lazy evaluation in the rest of paper.}

Although the calculation process of transformation is not visible to develoeprs, Spark can see all the methods that need to be calculated through this mode, and integrate the methods into different stages to execute, and achieve the best performance.

For DataFrame, all methods for data processing are transformation. The methods that are used to do basic data processing on the dataframe are: \texttt{Filter}, \texttt{dropDuplicates}, \texttt{distinct}, \texttt{distinct}, \texttt{dropna}, \texttt{fillna}, \texttt{drop}, \texttt{join}, \texttt{withColumn}, \texttt{sort}.

Deduplication can effectively reduce the data set and simplify the data set to improve performance. The \texttt{dropDuplicates} and \texttt{distinct} both will return a new DataFrame with duplicate rows removed. The difference is that \texttt{dropDuplicates} can deduplication based on the selected columns. \texttt{dropna} and \texttt{fillna} are essential methods in data cleaning. \texttt{dropna} will return a new DataFrame with removing the rows having null value. \texttt{fillna} will return a new DataFame with fillin the null value using selected value. The \texttt{drop} will return a new DataFrame that drops the selected columns. \texttt{join} is also a frequently used method in Spark. \texttt{join} will join two DataFrame based on the assigned condition. \texttt{withColumn} will returns a new DataFrame by adding a column. If the name of new column is same as the old one, the new column will replace the existing column that has the same name. \texttt{withColumn} is the most common method for data processing on spark. Because the dataframe is immutable, developers who want to perform any operation on a column of data in the dataframe need to use this method. \texttt{sort} will returns a new DataFrame that is sorted by the assigned columns.
\end{comment}


==> texFiles/discussion.tex <==
%\peter{I think we should have a discussion section that talks about the limitation of the approach, and we can even discuss the debug mode here. Also, what is the advantages of using breakpoints, and why our approach is different from breakpoints. What kind of benefits we can provide (e.g., production monitoring). Perhaps, we can also discuss user feedback here?}

\phead{Implications of Our Study.}
Below, we discuss the insights that we observed in our analysis on Stack Overflow posts and user study. Although the observations are related to data processing in Spark, the experience may be applicable to future research and development of tools for other big data applications.

\noindent{\em Knowing the intermediate information of data is important for debugging data processing applications.} In our user study, for the tasks where the participants are not allowed to use \tool, we observe that some participants tried to analyze Spark's logs and use Spark's cloud resource monitoring tool to debug the programs. However, even if the participants knew that there exists some issues in the program, they could not identify the root causes using the existing approaches. In most cases, the participants found that manually printing the data state (e.g., calling \texttt{print}) is the only useful approach for debugging. Some participants kept decomposing the chained methods, printing the output of each individual method, and checking for potential issues. Although we found that there were less manually-added print statements when the participants use a Python debugger, they still need to continuously decompose the chained methods to manually debug the result of each data processing method. More importantly, for the tasks in which \tool is not used, even after the participants found the issue, they still need to conduct extra analysis to find the root cause of the issue in the programs.
Different from existing debugging supports, \tool provides the intermediate information of data processing methods, which helps avoid decomposing the chained methods and reduce debugging effort. For instance, one participant mentioned that ``\emph{The information provided by the tool is very useful and precise. I can find the reason of the problem much quicker based on the given information.}'' Another participant mentioned that ``\emph{The tool is significantly better than printing information from the code. The information provided by the tool is quite rich and helpful for locating the problem.}'' Another participant mentioned, ``\emph{The tool is very easy to use and provides useful information without manual debugging.}'' We also observe that in 86.7\% of the tasks in which \tool is used, participants successfully identified the cause of the issue, which is much higher than that of the tasks in which \tool is not used(70\%). In other words, providing the intermediate information does help participants identify an issue and its root cause.




%from our analysis on how to improve the practice in debugging Spark application. Although these observations are obtained from our experience on \tool, they may be applicable to other development and debugging tools for big data applications and can be used to guide the future development of these tools.

%{\em Knowing the intermediate information of data is important for debugging data processing applications.} In our user study, for the tasks that are not allowed to use \tool, we observe that in some cases participants used the logging or web UI monitor that comes with Spark to debug, however it is still difficult for them to identify the issue, even if the participants knew that there exists an issue in the program and in the end they gave up using the tool coming with Spark. In most of the cases, printing the state of the data is the only useful method for debugging. We also observe that participants kept splitting the chained methods, printing the output of each individual function, and checking for issues. The situation gets better when using a debugger. But participants still need to continuously split the chained methods manually and debug each function to find the problem.



%Different from existing supportive tools, \tool provides intermediate information of data and avoids splitting the chained methods and manual debugging. For instance, one participant mentioned ``\emph{The information provided by the tool is very useful and precise, I can find the reason of the problem much quicker based on the given information.}'' One participant said ``\emph{The tool is significantly better than printing information from the code. The information provided by the tool is quite rich and helpful for locating the problem.}'' Another participant said ``It is very easy to use and provides useful information without manual debugging.''
%We observe that in \sw{rate?}\% of the tasks in which \tool is used, participants successfully identified the cause of the issue, which is much higher than that of the tasks in which \tool is not used. In other words, providing the intermediate information does help participants identify an issue and its root cause.


%Therefore, we call the errors and causes in the data processing process that participants find in the process of using traditional debugging tools as {\em Invisible problems and reasons.}

\noindent{\em Providing hints on anomalous data processing result helps identify issues more quickly.} As discussed in Section~\ref{sec:methodology}, \tool analyzes the execution of data processing methods and the value of their optional input parameters. If there is any anomalous result, \tool would provide a hint message. In our user study, we observe that such hints are useful for participants to notice the existence of an issue in the program. For example, one participant mentioned,``\emph{the most promising advantage of the tool is it can alarm users for anomalous behavior.}'' Another participant mentioned. Through these hints, it is easier for developers to quickly locate the abnormal behavior of the method or abnormal data.






%A participant said "Developers could easily find which step cause wrong data. This saves a lot of time."  Secondly, The information provided by \tool is closely related to function processing. When a developer generates a bug in the process of using these functions, this information is very effective for locating the problem. An participant said \wang{choose one} In addition, \tool will analyze the process of function execution and the input parameters of the function to check for abnormal behaviors to provide developers with effective information. A participant said "my feeling, the most promising advantage of the tool is it can alarm users for abnormal behavior". Different participants have different focuses on our tool. Fors the primary developers of Spark, they prefer the tool to provide status information and parameter hints for data processing. For experienced developers, they prefer the detection function of abnormal behavior provided by the tool.
%With help of our design, we can divide the help our tools bring to developers in two ways:quick and effective. First of all, our tool displays useful information about each function operation in the data processing process to the developer. Developers can quickly find errors in the data processing process by using \tool.

%\subsection{Implication}
%Now developers can \tool to understand their data processing programs. They do not need to worry about their data size and the performance of their programs. They can use \tool easily to understand their functions's output and avoid the potential problem in data processing functions. Moreover, when developers find their data processing function fails in cluster, they do not need to seperate their method-chaining and rerun their problem based on the original data and do a series of debugging job. Now they can benifit from \tool, which will can help develoeprs to locate problem quickly and effectively.

\phead{Limitations and Future Work.}
Our study provides an initial step towards understanding the data processing execution. Even though our findings show that the overhead of \tool is small and it can assist developers with debugging, there are still some limitations and future research opportunities in assisting the development of big data applications.

\noindent{\em Data Visualization and Information Presentation.} One common suggestion from the participants is related to improving the UI design. Currently, \tool records the intermediate information and hint messages in the form of text (e.g., similar to logs) without providing a rich user interface. A participant said, ``\emph{It would be perfect if the tool can finally come as an interactive form.}'' Another participant said ``\emph{it is hard to find the warning message and useful tips. I would suggest making the warning and tips easier to identify.}'' In addition to UI design, we also observed that visualizing the results of the data processing methods may also help developers quickly identify issues and understand the data state. For example, we find that in certain cases, some participants wanted to visualize the data using histograms to understand how the data distribution changes. Therefore, future studies may also consider leveraging data visualization to assist developers with developing and debugging big data applications.


\noindent{\em Customizable Information Recording.} Currently, \tool records all the data processing information that is described in Table~\ref{tab:req}. However, sometimes developers may already have an idea about possible issues that may occur, and they only want to record certain information. For example, in our user study, a participant mentioned that \emph{there is too much log information and it is not easy to locate the log I need immediately}. The participant is a professional developer who has years of experience in developing Spark applications. Even though the participant found \tool to be useful (gave \tool 5/5 in terms of usefulness), he suggested a customizable configuration for recording only the needed data processing information. Due to the vast amount of data and the complexity of big data applications, future studies may investigate approaches, such as providing a domain-specific language, that allows developers to record more customized and focused information to further assist debugging.


\noindent{\em More Advanced Debugging Assistance.} We uncover common challenges that developers encounter by analyzing questions on Stack Overflow. We then design an approach, \tool, and evaluate it by conducting a user study. Although our user study shows promising results, there is still other information that can be added to assist developers. For example, future studies may investigate more advanced techniques for providing hint messages for anomalous data processing results using machine learning or artificial intelligence. Moreover, to reduce the overhead of \tool, we apply random sampling to select a statistically significant subset of data. Although sampling is an effective technique to reduce the data size while providing good precision on the original, future studies may investigate different sampling techniques and how they affect the effectiveness of debugging big data applications. % data representation in the samples.



%{\em Abnormal behaviour analysis.} For the abnormal detection, we can tell developers which function has abnormal behaviour. There are more things we can do. In the future work, we will analyze the abnormal behavior, not to tell the developer which functions are currently problematic, but to provide the developer with the cause of the problem.


%{\em Better sampling ways.} The current overhead of \tool is mainly on initial sampling. Although this overhead can be gradually ignored as the data scaled, and it will not increase linearly with the data scaled, future work should continue to optimize the sampling method, such as increasing the index to reduce the overhead.


==> texFiles/related.tex <==
%\sw{may need a better name}\h{how about: Understanding the challenges of developing big-data applications}
\phead{Understanding the Challenges of Developing Big Data Applications.} 
%{\em Research on big data challenge.}
%To process massive amount of data in the cloud, developers leverage big data processing frameworks such as Google’s MapReduce~\cite{mapreduce}, Hadoop~\cite{hadoop}, and Spark~\cite{spark}. Developers may encounter various problems when using such frameworks. 
Prior studies have been done to understand the challenges that developers encounter. %Fisher et al.~\cite{fisher2012interactions} find that debugging for a cloud-based computation solution is more challenging compared to debugging on a single machine. %, e.g., developers often find themselves digging through trace files distributed across multiple virtual machines to debug issues. 
Bagherzadeh et al.~\cite{Bagherzadeh:2019:GBL:3338906.3338939} mined Stack Overflow questions to understand the big data-related questions that developers ask. They find that developers ask questions about MapReduce model, debugging, and basic concepts more frequently than questions about performance. Kim et al.~\cite{8046093} surveyed 793 Microsoft data scientists on the common challenges that they encounter. They find that the most common challenges are related to data quality and the scale of the data. Fisher et al.~\cite{fisher2012interactions} also interviewed 16 data analysts at Microsoft and they found that debugging in a distributed cloud environment is extremely challenging. 
Zhou et al.~\cite{10.5555/2819009.2819014} analyzed 210 issue reports from one of Microsoft's big data platforms. They find that more than 30\% of the issues are related to application design and code logic. In this paper, we focus our qualitative study on Stack Overflow questions related to Spark development. Similarly, we find that the most common questions that developers encounter are related to data processing and debugging. We then design an approach aiming to assist developers with such challenges. 




%Beller et al.~\cite{10.1145/3180155.3180175} found that only 23\% research subjects actively use IDE-provided debuggers, while 72.2\% research subjects would like to examine log files and 71.6\% research subjects still use \texttt{print} statement to debug.


%\sw{consider cut this, the paper is about general debugging, not about big data applications}
%Although a few debugging tools have been developed to support the debugging with big data processing framework, Beller et al.~\cite{10.1145/3180155.3180175} found that only 23\% research subjects actively use IDE-provided debuggers, while 72.2\% research subjects would like to examine log files and 71.6\% research subjects still use \texttt{print} statement to debug. Their research shows both knowledge and use of advanced debugging features are low. Their results echo our observation in the user study that in most cases, the participants found that manually printing the data state (e.g., calling \texttt{print}) is the only useful approach for debugging. %Several studies reveal that configuring a big data processing framework for optimizing its performance is a challenge task~\cite{li2014adaptive}.



%\sw{may need a better name}
\phead{Supporting Debugging for Big Data Processing Applications.} 
%To support the debugging of applications using big data processing frameworks, a number of research endeavor has been made. 
%Prior studies aim to provide debugging supports for big data processing frameworks. 
Dave et al.~\cite{Dave2013ArthurR} proposed Arthur, which is a debugger for Hadoop and Spark. Arthur enables a user to selectively replay a part of the original computation with low overhead. However, it does not support the inspection of intermediate information at runtime. Gulzar et al.~\cite{10.1145/2884781.2884813,gulzar2017automated,10.1145/3236024.3264586,10.1145/3338906.3338953} developed a series of techniques to support the debugging and testing for big data applications. Gulzar et al. proposed BIGDEBUG~\cite{10.1145/2884781.2884813}, which is a debugger for Spark applications without needing to interrupt or re-run Spark applications during debugging. %BIGDEBUG can stimulate breakpoints in Spark applications, which allows developers to check their intermediate data results. It can also provide the location of a crash-including record and resume the related computation after the problem is fixed.
%BIGDEGUG provides developers with a way to debug Spark application without interrupting or re-running Spark applications.
However, BIGDEBUG modifies the Spark source code and only supports the legacy RDD APIs, which limits the adoption of this tool as some developers or companies may not be willing to replace the official Spark implementation with third-party customized Spark. %In addition, BIGDEBUG only supports the legacy RDD APIs. %It does not support the currently common API in Spark, such as DataFrame and DataSet. 
Different from BIGDEBUG, we apply the Adapter design pattern to \tool and implement it as a package so that developers barely need to modify their existing source code when using \tool. Instead of setting up breakpoints for debugging, we provide the intermediate state of data and also provide hints for anomalous data processing results and API parameters, which have low overhead and are demonstrated to be useful in helping identify issues through our user study. %\sw{does bigdebug support debugging for chained method? if not we should highlight it.}
Gulzar et al. developed BigSift~\cite{10.1145/3236024.3264586, gulzar2017automated}, which is a tool for finding the root cause of an error due to an unclean dataset or a wrong assumption of the data. BigSift combined delta debugging and data provenance to provide a Web interface for locating wrong input records in a Spark application. Different from these work, \tool focuses on providing an intermediate state of data in chained methods and providing hints for anomalous data processing results.
%They also developed BigTest~\cite{10.1145/3338906.3338953}, which is a new white-box testing technique that can achieve the same code coverage as the entire data by generating a small test dataset. They show that BigTest detects more faults and consumes less CPU time.
%
%Another line of research is focusing on debugging by analyzing logs~\cite{shang2013assisting,tan2008salsa,xu2009detecting}. For instance, Shang et al. proposed an approach to detect the deployment failures by comparing the execution log captured on the cloud with the log captured using a local mode. Different from this line of work, we generate logs that provide intermediate information of data and hints for anomalous data processing result.



%\sw{I would drop them, there are not related to big data}
%Reactive programming is programming with asynchronous data streams. Traditional debug tools lack support for Reactive Programming.  “RP Debugging” ~\cite{10.1145/2884781.2884815} is a debugger model for the REScala~\cite{inproceedings} that is a reactive programming library for Scala. This debugger integrates with Eclipse IDE to provide Scala developers the dependency graph visualization, reactive breakpoint and performance monitoring. Benken et al.~\cite{10.1145/3180155.3180156} proposed a visualization and debugging tool targeted to Rx. The dependencies and structure of the data flow in program can be visualized. This debugger can work on different programming languages and outside of the IDE.
%For debugging in Spark, Spark official support Web Ui monitor, which can observe the execution process of the program in a visual form.
%Omniscient Debugging~\cite{10.1109/MS.2009.169} can provide developers track down the root cause of bugs easily by exploring program's execution history. However, the performance may be a problem as there may be too much program execution information to be computed.



==> texFiles/rq1.tex <==
\subsection*{RQ: What is the performance overhead of our approach?}
\phead{Approach.} We implement six Spark benchmarking programs for our experiment. To measure the scalability of our approach, we run each program using three different levels of data size: 50MB, 500MB, and 5GB. We follow prior studies~\cite{10.1145/2491894.2464160, 10.1145/1297027.1297033, peter_orm} and repeat each performance measurement 20 times.

\phead{Preliminary Results.} The overhead of our approach is around 1 to 3 seconds for 50MB data and 6 to 8 seconds for 5GB data and the ratio of the overhead decreases as the data size increases. The preliminary results shows the overhead of our approach is consistent across programs, and the overhead remains stable even when the data size is increased by 100 folds (i.e., from 50MB to 5GB). Our initial finding shows that our approach has a good scalability. 










==> texFiles/threats.tex <==
%{\em } At present, \tool also support the python language, and we do not cover all the APIs for data processing. Developers may generate errors in APIs that we have not covered. Spark developers who use Scala and Java cannot use \tool. In the future, we will extend our api and support Scala and Java languages.


\noindent\textbf{External validity.} Threats to external validity relate to the generalizability of our findings. In Section~\ref{sec:motivation}, we studied the Spark-related questions on Stack Overflow. % to understand the challenges that developers encounter when developing Spark applications. 
The number of questions is large and it is impossible to study all of the questions qualitatively. To minimize the bias, we randomly sampled 1,000 statistically representative questions, giving a confidence level of 95\% and a
confidence interval of 3\%. We implement \tool to support Spark's Python version. Our findings may not be generalized to Spark APIs in Java and Scala. However, our proposed methodology could be easily applied to the other two languages and future research is encouraged to enhance the support for other programming languages.
Similarly, we do not cover all the APIs for data processing. However, in this study, we cover all the basic data processing APIs for PySpark's DataFrame~\cite{pysparkAPI} and our user study demonstrates that \tool is effective in helping developers identify issues and their root causes. Future research is encouraged to apply our approach to other data processing APIs.

\noindent\textbf{Internal Validity.} Threats to internal validity are related to experimenter errors and bias. We conducted a qualitative study in Section~\ref{sec:motivation} which was performed by humans and bias may be introduced. To reduce the bias, each question is examined by two of the authors individually and discrepancies are discussed until a consensus is reached. We measured the level of the inter-rate agreement in our qualitative study, and the agreement value is high (i.e., 0.825). % even before the consensus is reached. 
